Free Process Rewards without Process Labels

Different from its counterpart outcome reward models (ORMs), which evaluate the entire responses, a process reward model (PRM) scores a reasoning trajectory step by step, providing denser and more fine grained rewards. However, training a PRM requires labels annotated at every intermediate step, presenting significant challenges for both manual and automatic data collection. This paper aims to address this challenge. Both theoretically and empirically, we show that an \textit{implicit PRM} can be obtained at no additional cost, by simply training an ORM on the cheaper response-level labels. The only assumption is to parameterize the outcome reward as the log-likelihood ratios of the policy and reference models, which can be optimized regardless of the specific choice of loss objectives. In experiments, we instantiate our implicit PRMs with various objectives and evaluate their performance on MATH. We show that our implicit PRM outperforms a strong MCTS-based baseline \textit{\'a la} Math-Shepherd using less than $1/38$ of the training data. Its performance can be further improved with majority voting. We further find that scaling up instructions and responses benefits our implicit PRM, and the latter brings a larger gain. Particularly, we find that our implicit PRM, when instantiated with the cross-entropy (CE) loss, is more data-efficient and can keep improving generation models even when trained with only one response per instruction, the setup that suffers from extreme data scarcity and imbalance. Further, instructions should be relevant to downstream tasks while the diversity of responses does not bring gains. Surprisingly, training on extra Math-Shepherd step labels brings no further improvements to our implicit PRM trained on only outcome data. We hope that our work will encourage a rethinking of PRM training approaches and contribute to making training PRMs more accessible.

==> fig_tex/loss.tex <==
\begin{figure}[tbh]
    \centering
    % \includegraphics[width=0.32\linewidth]{figs/losses_Mistral-7B-Inst-v0.2.pdf}
    % \includegraphics[width=0.32\linewidth]{figs/losses_Llama-3.1-8B-Inst.pdf}
    % \includegraphics[width=0.32\linewidth]{figs/losses_Llama-3.1-70B-Inst.pdf}
    \includegraphics[width=\linewidth]{figs/losses.pdf}
    \caption{Instantiating our implicit PRMs with different training objectives. DPO and NCA are trained on pairwise data while KTO and CE are not. CE (Balanced) down samples rollouts to each instruction to balance the positive and negative ones. Results show that DPO works the best\hao{same suggestion as in the text}, and balancing positive and negative data is beneficial to implicit PRM.\lifan{this means we still need paired data, which is awkward}
    }
    \label{fig:loss}
\end{figure}

==> fig_tex/method_comparison.tex <==
\begin{figure}[tbh]
    \centering
    % \includegraphics[width=0.32\linewidth]{figs/method_comparison_Mistral-7B-Inst-v0.2.pdf}
    % \includegraphics[width=0.32\linewidth]{figs/method_comparison_Llama-3.1-8B-Inst.pdf}
    % \includegraphics[width=0.32\linewidth]{figs/method_comparison_Llama-3.1-70B-Inst.pdf}
    \includegraphics[width=\linewidth]{figs/method_comparison.pdf}
    \caption{Comparison with baselines on best-of-N. Our implicit PRM consistently outperforms baselines given different numbers of solutions to each problem.}
    \label{fig:main-exp}
\end{figure}

==> fig_tex/prm_pilot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.32\linewidth]{figs/accuracy_trend_positive.pdf}
    \includegraphics[width=0.32\linewidth]{figs/accuracy_trend_negative.pdf}
    \includegraphics[width=0.32\linewidth]{figs/accuracy_trend_all.pdf}
    \caption{Caption}
    \label{fig:prm-sampling}
\end{figure}

==> tab_tex/loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\caption{Different Objectives \lifan{also present policy performance}\ganqu{suggest making a fig}}
\label{tab:loss}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|c|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{2}{*}{Objective} & \multirow{2}{*}{\# Resp} & \multicolumn{5}{c|}{Llama-3.1-8b-inst} & \multicolumn{5}{c|}{Llama-3.1-70b-inst} & \multicolumn{5}{c}{Eurux-8x22b-nca} \\ \cmidrule(l){3-17} 
                           &                          & @1     & @8    & @16   & @32   & @64   & @1     & @8     & @16   & @32   & @64   & @1  & @8    & @16   & @32   & @64   \\ \midrule
DPO                        & \multirow{4}{*}{8}       & 44.6   & 54.6  & 55.6  & 55    & 56.6  & 47.6   & 56.2   & 57.6  & 59    & 59.6  & 46  & 55.1  & 55    & 57.2  & 56.6  \\
KTO                        &                          & 44.6   & 52.2  & 51.8  & 52.4  & 50.8  & 47.6   & 55.8   & 54.2  & 53.6  & 51.8  & 46  & 51.8  & 51.2  & 51.2  & 52    \\
NCA                        &                          & 44.6   & 53.2  & 53.4  & 53.6  & 55.2  & 47.6   & 54.4   & 56.6  & 56.4  & 55.6  & 46  & 53.2  & 53.6  & 53.2  & 54.4  \\
CE                         &                          & 44.6   & 55    & 55.4  & 54    & 55.4  & 47.6   & 54.8   & 55.4  & 58    & 58.2  & 46  & 55.2  & 56    & 53.8  & 55    \\ \bottomrule
\end{tabular}
}
\end{table}

==> tab_tex/sampling_acc.tex <==
% \begin{wraptable}{r}{0.5\linewidth}
% \caption{sampling acc}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccc}
%         \toprule
%         \multirow{2}{*}{Method} & \multicolumn{3}{l}{Accuracy On Different Labels} \\ \cline{2-4} 
%                                 & Positive        & Negative        & All          \\ \midrule
%         All Annotated           & 62.30           & 64.81           & 63.55        \\
%         Lean To Negative        & 57.15           & \textbf{67.90}           & 62.52        \\
%         Lean To Positive        & \textbf{72.72}           & 64.81           & \textbf{68.76}        \\ \bottomrule
%         \end{tabular}
% }
% \end{wraptable}
\begin{wraptable}{r}{0.35\linewidth}
\caption{Accuracy of different step label estimation strategy.}
\label{tab:sampling_acc}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
        \toprule
        Method & Accuracy \\ \midrule 
        All Annotated           & 63.55        \\
        Lean To Negative        & 62.52        \\
        Lean To Positive        & \textbf{68.76}        \\ \bottomrule
        \end{tabular}
}
\end{wraptable}

==> tab_tex/tokens.tex <==
\begin{wraptable}{r}{0.65\textwidth}
\centering
\caption{Tokens consumption of different approaches.}
\label{tab:tokens}
\resizebox{0.6\textwidth}{!}{

\begin{tabular}{@{}lc|cc|cc|c@{}}
\toprule
\multicolumn{2}{l|}{Stage}                             & \multicolumn{2}{c|}{Step Label Annotation} & \multicolumn{2}{c|}{PRM Training} & \multirow{2}{*}{Total} \\ \cmidrule(r){1-6}
\multicolumn{1}{l|}{Method}                  & \# Resp & Input                & Output              & Input           & Output          &                        \\ \midrule
\multicolumn{1}{l|}{\multirow{4}{*}{MCTS}}   & 1       & 2443.1M              & 162.8M              & 3.2M            & 10.5M           & 2619.6M                \\
\multicolumn{1}{l|}{}                        & 2       & 4882.3M              & 325.1M              & 6.3M            & 21.0M           & 5234.7M                \\
\multicolumn{1}{l|}{}                        & 4       & 9764.3M              & 650.8M              & 12.7M           & 41.9M           & 10469.7M               \\
\multicolumn{1}{l|}{}                        & 8       & 19519.0M             & 1300.5M             & 25.3M           & 83.8M           & 20928.6M               \\ \midrule
\multicolumn{1}{l|}{\multirow{4}{*}{AutoPSV}} & 1       & 47.6                 & 0.2M                & 50.8M           & 10.6M           & 109.2M                 \\
\multicolumn{1}{l|}{}                        & 2       & 95.1M                & 0.3M                & 101.4M          & 21.2M           & 218.0M                 \\
\multicolumn{1}{l|}{}                        & 4       & 190.1M               & 0.6M                & 202.8M          & 42.4M           & 435.9M                 \\
\multicolumn{1}{l|}{}                        & 8       & 380.1M               & 1.2M                & 405.4M          & 84.8M           & 871.5M                 \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{DPO}}    & 2       & 0                    & 0                   & 1.6M            & 5.6M            & 7.2M                   \\
\multicolumn{1}{l|}{}                        & 4       & 0                    & 0                   & 9.4M            & 32.9M           & 42.3M                  \\
\multicolumn{1}{l|}{}                        & 8       & 0                    & 0                   & 44.2M           & 154.1M          & 198.3M                 \\ \bottomrule
\end{tabular}

}
\vspace{-10pt}
\end{wraptable}
